MG/OPT and MLMC for Robust Optimization of PDEs

An algorithm is proposed to solve robust control problems constrained by partial differential equations with uncertain coefficients, based on the so-called MG/OPT framework. The levels in this MG/OPT hierarchy correspond to discretization levels of the PDE, as usual. For stochastic problems, the relevant quantities (such as the gradient) contain expected value operators on each of these levels. They are estimated using a multilevel Monte Carlo method, the specifics of which depend on the MG/OPT level. Each of the optimization levels then contains multiple underlying multilevel Monte Carlo levels. The MG/OPT hierarchy allows the algorithm to exploit the structure inherent in the PDE, speeding up the convergence to the optimum. In contrast, the multilevel Monte Carlo hierarchy exists to exploit structure present in the stochastic dimensions of the problem. A statement about the rate of convergence of the algorithm is proven, and some additional properties are discussed. The performance of the algorithm is numerically investigated for three test cases. A reduction in the number of samples required on expensive levels and therefore in computational time can be observed.

==> fig/prob1/p2mlmc/Ey.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[baseline=(img)]
\node (img) at (0,0) {\includegraphics[width=\figurewidth]{fig/prob1/p2mlmc/Ey.jpg}};
\useasboundingbox ([xshift=-0.08\figurewidth]current bounding box.south west) rectangle ([xshift=-0.08\figurewidth]current bounding box.north east);
%\draw (current bounding box.south west) rectangle (current bounding box.north east);
\node [align=center] at (0.32\figurewidth,-0.3\figureheight){$x_1$};
\node [align=center] at (-0.35\figurewidth,-0.27\figureheight){$x_2$};
\node [align=center,rotate=90] at (-0.55\figurewidth,0.05\figureheight){$\mean{y}$};
\end{tikzpicture}%

==> fig/prob1/p2mlmc/Vy.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[baseline=(img)]
\node (img) at (0,0) {\includegraphics[width=\figurewidth]{fig/prob1/p2mlmc/Vy.jpg}};
\useasboundingbox ([xshift=-0.08\figurewidth]current bounding box.south west) rectangle ([xshift=-0.08\figurewidth]current bounding box.north east);
%\draw (current bounding box.south west) rectangle (current bounding box.north east);
\node [align=center] at (0.32\figurewidth,-0.3\figureheight){$x_1$};
\node [align=center] at (-0.35\figurewidth,-0.27\figureheight){$x_2$};
\node [align=center,rotate=90] at (-0.55\figurewidth,0.05\figureheight){$\var{y}$};
\end{tikzpicture}%

==> fig/prob2/p1mlmc/Ey.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[baseline=(img)]
\node (img) at (0,0) {\includegraphics[width=\figurewidth]{fig/prob1/p1mlmc/Ey.jpg}};
\useasboundingbox ([xshift=-0.08\figurewidth]current bounding box.south west) rectangle ([xshift=-0.08\figurewidth]current bounding box.north east);
%\draw (current bounding box.south west) rectangle (current bounding box.north east);
\node [align=center] at (0.32\figurewidth,-0.3\figureheight){$x_1$};
\node [align=center] at (-0.35\figurewidth,-0.27\figureheight){$x_2$};
\node [align=center,rotate=90] at (-0.55\figurewidth,0.05\figureheight){$\mean{y}$};
\end{tikzpicture}%

==> fig/prob2/p1mlmc/Vy.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[baseline=(img)]
\node (img) at (0,0) {\includegraphics[width=\figurewidth]{fig/prob1/p1mlmc/Vy.jpg}};
\useasboundingbox ([xshift=-0.08\figurewidth]current bounding box.south west) rectangle ([xshift=-0.08\figurewidth]current bounding box.north east);
%\draw (current bounding box.south west) rectangle (current bounding box.north east);
\node [align=center] at (0.32\figurewidth,-0.3\figureheight){$x_1$};
\node [align=center] at (-0.35\figurewidth,-0.27\figureheight){$x_2$};
\node [align=center,rotate=90] at (-0.55\figurewidth,0.05\figureheight){$\var{y}$};
\end{tikzpicture}%

==> fig/prob3/p1mlmc/Ey.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[baseline=(img)]
\node (img) at (0,0) {\includegraphics[width=\figurewidth]{fig/prob1/p1mlmc/Ey.jpg}};
\useasboundingbox ([xshift=-0.08\figurewidth]current bounding box.south west) rectangle ([xshift=-0.08\figurewidth]current bounding box.north east);
%\draw (current bounding box.south west) rectangle (current bounding box.north east);
\node [align=center] at (0.32\figurewidth,-0.3\figureheight){$x_1$};
\node [align=center] at (-0.35\figurewidth,-0.27\figureheight){$x_2$};
\node [align=center,rotate=90] at (-0.55\figurewidth,0.05\figureheight){$\mean{y}$};
\end{tikzpicture}%

==> fig/prob3/p1mlmc/Vy.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[baseline=(img)]
\node (img) at (0,0) {\includegraphics[width=\figurewidth]{fig/prob1/p1mlmc/Vy.jpg}};
\useasboundingbox ([xshift=-0.08\figurewidth]current bounding box.south west) rectangle ([xshift=-0.08\figurewidth]current bounding box.north east);
%\draw (current bounding box.south west) rectangle (current bounding box.north east);
\node [align=center] at (0.32\figurewidth,-0.3\figureheight){$x_1$};
\node [align=center] at (-0.35\figurewidth,-0.27\figureheight){$x_2$};
\node [align=center,rotate=90] at (-0.55\figurewidth,0.05\figureheight){$\var{y}$};
\end{tikzpicture}%
